A Survey on Retrieval-Augmented Text Generation

Recently, retrieval-augmented text generation attracted increasing attention of the computational linguistics community. Compared with conventional generation models, retrieval-augmented text generation has remarkable advantages and particularly has achieved state-of-the-art performance in many NLP tasks. This paper aims to conduct a survey about retrieval-augmented text generation. It firstly highlights the generic paradigm of retrieval-augmented generation, and then it reviews notable approaches according to different tasks including dialogue response generation, machine translation, and other generation tasks. Finally, it points out some important directions on top of recent methods to facilitate future research.

==> A Comprehensive Survey on Retrieval based Text Generation Methods/sec-conclusion.tex <==
In this paper, we surveyed recent approaches for retrieval-augmented text generation. We reviewed and summarized the development of different components of retrieval-augmented text generation including retrieval metrics, retrieval sources, and integration paradigms. We gave in-depth discussions when retrieval-augmented text generation comes to different applications including dialogue response generation, machine translation, and other generation tasks. We also pointed out some future directions for retrieval-augmented text generation. 

==> A Comprehensive Survey on Retrieval based Text Generation Methods/sec-dialogue-generation.tex <==
\paragraph{Background} Dialogue systems can be grouped into two categories: chit-chat systems and task-oriented systems. While task-oriented dialogue systems are designed to accomplish specific user tasks such as air tickets booking, chit-chat dialogue systems aim at giving a meaningful and fluent response for any dialogue history in the open domain. Dialogue response generation in chit-chat dialogue system is challenging partly due to the diversity of possible responses to a single dialogue history (i.e., the \textit{one-to-many} problem). The dialogue history alone cannot decide a meaningful and specific response. Also, external knowledge that is not present in the dialogue history are often necessary for avoiding safe but boring responses. We focus on recent efforts tackling the challenges to develop chit-chat dialogue systems.

Most modern chit-chat dialogue systems can be categorized into two classes, namely, retrieval-based models and generation-based models. The retrieval-based models  \cite{ji2014information,hu2014convolutional} directly copy an existing response from curated dialogue corpora (i.e., the retrieval pool) when receiving a response request. The retrieved responses are often informative and grammatical as they are collected from real-world conversations and possibly post-edited by a human. However, such systems perform poorly when a given dialogue history is substantially different from those in the retrieval pool. On the other hand, the generation-based models \cite{shang-lu-li:2015:ACL-IJCNLP,vinyals2015neural,li-EtAl:2016:N16-11} generate a new utterance from scratch. Those generation-based models have better generalization capacity when handling unseen dialogue contexts. Nevertheless, the generated utterances are inclined to be dull and non-informative (e.g., ``I don't know'', ``I think so'', ``Me too'' etc.) \cite{li-EtAl:2016:N16-11}.

\paragraph{Shallow Integration} As discussed, retrieval-based models may give informative but inappropriate responses while generation-based models often do the opposite. It is desirable to combine the best of both worlds. Early work \cite{qiu-EtAl:2017:Short} attempts to re-rank the output from both models. For a deep integration, \newcite{song2016two} and \newcite{yang2019hybrid} extend the standard \textsc{Seq2Seq} encoder-decoder model \cite{bahdanau2014neural} with an extra encoder for encoding the retrieval result. The output of the extra encoder, along with the output from the original encoder for dialogue history, is used to feed the decoder. \newcite{weston-etal-2018-retrieve} use a single encoder that takes the concatenation of the original dialogue history and the retrieved as input. \newcite{wu2019response} note that the retrieved information should be used in awareness of the context difference, and further proposed to construct an edit vector by explicitly encoding the lexical differences between the input dialogue history and the retrieved dialogue history. \newcite{pandey2018exemplar} further propose to weight different training instances by context similarity.

\paragraph{Deep Integration} To prevent the inflow of erroneous information, \newcite{cai2019skeleton} propose a general framework that first extracts a skeleton from the retrieved response and then generates the response based on the extracted skeleton. This framework is also adopted for stylistic response generation \cite{su2021prototype}. \newcite{gupta-etal-2021-controlling} suggest to use the semantic structure of an exemplar response, instead of the tokens of the exemplar response, to guide generation. Despite their differences, a common issue is that the generation model easily learns to ignore the retrieved response entirely and collapses to a vanilla seq2seq model. This happens with improper training instances. Due to the one-to-many nature, it happens frequently that a retrieved response (extracted skeleton) is suitable for responding to the query, but inconsistent with the current target response.

Earlier studies \cite{weston-etal-2018-retrieve,wu2019response,cai2019skeleton} alleviate the above problems by putting hard constraints on the data (e.g., discarding data with low similarity of the retrieved response and the target response), which, however, greatly reduces the amount of usable data. \newcite{cai-etal-2019-retrieval} employ a random mechanism for generating the skeletons used for training, which extract skeletons from the corresponding responses with some deliberate disturbance. \newcite{paranjape2021hindsight} propose to model the retriever after the posterior distribution of retrieval given the input and the target output and train it jointly with the standard retriever and the generator by maximizing the evidence lower bound (ELBo) in expectation over retrieval.

\paragraph{Knowledge-Enhanced Generation} The aforementioned work demonstrates that retrieval-based dialogue systems can be used for building better generation-based models. In general, this is done by conditioning the generation on some retrieved responses. More traditionally, to infuse the response with external knowledge, the retrieval pool is not necessarily a dialogue corpus. In fact, knowledge-grounded dialogue response generation exploring different forms of knowledge such as knowledge bases and external documents \cite{dinan2018wizard,zhou2018dataset,lian2019learning,li2019incremental,qin2019conversing,wu2021controllable,zhang2021joint,komeili2021internet} has been actively explored.

\paragraph{Limitations} We note that there are three major limitations in existing work for dialogue response generation. First, current methods only use one retrieved response for generation. It can be more beneficial to combine multiple retrieval responses. However, this can be difficult due to the one-to-many nature of dialogue response generation. Second, current methods use universal relevance score for retrieval. It can be more effective if we can use more customized retrieval metric especially for controlled dialogue response generation (e.g., persona, emotion, etc).  Third, the retrieval pool of existing methods is limited to dialogue corpora (context-response pairs) or documents. It might be useful to enlarge the retrieval pool by including more corpora in other domains or in other modalities. As discussed, there leaves plenty of possible directions to explore in the future. 



==> A Comprehensive Survey on Retrieval based Text Generation Methods/sec-future-research.tex <==

% \begin{table*}[]
%     \centering
%     \begin{tabular}{c|c|c|c|c|c}
%         Tasks & Ref. & Source & Metric & Integration  &  Model  \\
%          \hline
%          &  &  &  &   &    \\
%          \hline
%          Others&  &  &  &   &    \\
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:my_label}
% \end{table*}


%\subsection{Limitations}
Despite the current success of retrieval augmented text generation, there is still a long way to go as discussed in previous sections. We highlight some directions to facilitate the future research as follows:
\paragraph{Retrieval Sensitivity} The performance of retrieval augmented text generation is very sensitive to the retrieval quality, i.e., the similarity between the query and the retrieved examples. Currently, retrieval augmented text generation models perform well when the retrieved examples are very similar to the query. However, they are even worse than the generation models without retrieval when the retrieval examples are less similar. Therefore, it would be important to exploit new methods to address such an issue on similarity.
    % \cd{if space is limited, consider delete this point.} 
\paragraph{Retrieval Efficeincy} Generally, if one enlarges the retrieval memory to some extent, it would be possible to retrieve an example which is very similar to the query.% \cd{cannot understand? impossible $\Rightarrow$ possible?}.
    Unfortunately, the downside is that the overall inference for the retrieval augmented generation models is less efficient due the considerable retrieval overhead. In this sense, it is urgent to consider some methods to trade off the retrieval memory size and retrieval efficiency, for example, data compression for the retrieval memory.
\paragraph{Local vs. Global Optimization} Theoretically, it seems promising to jointly learn retrieval metrics and generation models. However, in practice, there is an essential gap about the retrieval metric between the training and inference phrases. In the training phase, the loss is locally back-propagated to only a few retrieved examples while in the inference phase the metric is globally conducted among all examples in the memory. It would be interesting to narrow such a gap when learning a better metric for generation tasks. 
    
 \paragraph{Multi-Modalities} With recent advancement in image-text retrieval, directly associating images with relevant text becomes possible. This urges researchers to investigate the possibility of retrieval-based text generation in tasks that involve data from different modalities. One typical task is image captioning. Beyond images, other tasks like speech-to-text transcription could potentially benefit from retrieval-based generation methods as well.
    
 \paragraph{Diverse \& Controllable Retrieval} Most of the existing approaches adopt a universal metric for retrieval, such as lexical similarities of sentences. Future work should explore how to use customized metrics for retrieval. This can be beneficial for more controlled text generation. For example, instances with emotions and styles may be more desirable in the personalized dialogue generation, parallel data that contains specific terminologies is more helpful in machine translation, and so on. On the other hand, using a universal metric for retrieval may lead to the lack of diversity of the retrieval results. Collecting a diverse set of retrieval results can improve the coverage of useful information. Thus, considering multiple different metrics for retrieval may lead to generation with higher quality in the future.


==> A Comprehensive Survey on Retrieval based Text Generation Methods/sec-introduction.tex <==
Retrieval-augmented text generation, as a new text generation paradigm that fuses emerging deep learning technology and traditional retrieval technology, has achieved state-of-the-art (SOTA) performance in many NLP tasks and attracted the attention of the computational linguistics community \cite{weston-etal-2018-retrieve,dinan2018wizard,cai-etal-2021-neural}. Compared with generation-based counterpart, this new paradigm has some remarkable advantages: 1) The knowledge is not necessary to be implicitly stored in model parameters, but is explicitly acquired in a plug-and-play manner, leading to great scalibility; 2) Instead of generating from scratch, the paradigm generating text from some retrieved human-written reference, which potentially alleviates the difficulty of text generation. 
%Although retrieval-augmented generation is promising, to the best of our knowledge, there is no survey  

% Recent developments in this paradigm are distributed \hyli{rewrite: Combining the pros of neural network and retrieval is becoming a new trend} in many sub-domains of text generation, such as dialogue response generation, machine translation, and style transfer. It demonstrates the universality of retrieval-augmented text generation but also increases the difficulty on understanding the underlying mechanism, especially for newcomers to get started. They are required to be not only familiar with recent work in both neural NLP and retrieval technology, but also aware of the characteristics of downstream tasks. A comprehensive survey may fill this gap and introduce the nascent field of retrieval-augmented text generation. \cd{I think we should focus more on the importance of the subject, not its complexity.}

This paper aims to review many representative approaches for retrieval-augmented text generation tasks including dialogue response generation~\cite{weston-etal-2018-retrieve}, machine translation~\cite{gu2018search} and others~\cite{hashimoto2018retrieve}. We firstly present the generic paradigm of retrieval-augmented generation as well as three key components under this paradigm, which are retrieval sources, retrieval metrics %~\cite{ramos2003using,JDH17} 
and generation models.%~\cite{bahdanau2014neural}
%, respectively. 
\begin{figure*}[h]     
  \center{\includegraphics[width=\textwidth] {Figures/Figure1.pdf}}        
  \caption{
  %The overview of our proposed end-to-end framework, which contains DR-BERT training and online inference procedures. $r_i$ denotes the $i$-th response. $c_i$ denotes the $i$-th multi-turn dialog history, and $c_{i,j}$ denotes the $j$-th utterance in $c_i$. $V_{r_i}$ denotes the semantic embeddings of $r_i$ that is generated by response BERT encoder BERT$_{res}$. During online inference, the corpus is nonparallel and consists of large amounts of single sentences. 
  %\textcolor{red}{branden: 
  The overview of this survey.}
  %}
  \label{img:overview}
\end{figure*}


Then, we introduce notable methods about retrieval-augmented generation, which are organized with respect to different tasks. Specifically, on the dialogue response generation task, exemplar/template retrieval as an intermediate step has been shown beneficial to informative response generation \cite{weston-etal-2018-retrieve,wu2019response,cai2019skeleton,cai-etal-2019-retrieval}. In addition, there has been growing
interest in knowledge-grounded generation exploring different forms of knowledge such as knowledge bases and external documents \cite{dinan2018wizard,zhou2018dataset,lian2019learning,li2019incremental,qin2019conversing,wu2021controllable,zhang2021joint}. 
%On the machine translation task, we summarize the early work on how the retrieved sentences (called translation memory) are used to improve statistical machine translation (SMT)~\cite{koehn-etal-2003-statistical} models~\cite{simard2009phrase,koehn2010convergence,liu2012locally}. Since neural machine translation (NMT)~\cite{bahdanau2014neural} delivers dominant advantages compared with SMT thanks to its end-to-end modeling and sufficient training data, in particular, we intensively highlight several popular methods to integrating translation memory to NMT models~\cite{gu2018search,zhang2018guiding,xu2020boosting,he2021fast, cai-etal-2021-neural}. 
On the machine translation task, we summarize the early work on how the retrieved sentences (called translation memory) are used to improve statistical machine translation (SMT)~\cite{koehn-etal-2003-statistical} models~\cite{simard2009phrase,koehn2010convergence} and in particular, we intensively highlight several popular methods to integrating translation memory to NMT models~\cite{gu2018search,zhang2018guiding,xu2020boosting,he2021fast}. 
We also review the applications of retrieval-augmented generation in other generation tasks such as abstractive summarization \cite{peng2019text}, code generation \cite{hashimoto2018retrieve}, paraphrase \cite{kazemnejad-etal-2020-paraphrase,su-etal-2021-keep}, and knowledge-intensive generation \cite{lewis2020retrieval}. 
Finally, we also point out some promising directions on retrieval-augmented generation to push forward the future research. %\hyli{Do we need to compress this paragraph? It is a little bit heavy now, and the the connection between this paragraph and the previous one is not that good.}

==> A Comprehensive Survey on Retrieval based Text Generation Methods/sec-machine-translation.tex <==
Retrieval augmented translation originates from human translation scenarios~\cite{somers2003translation}. When translating $\hat{\boldsymbol{y}}$ from an input source sentence $\boldsymbol{x}$, a human translator typically involves a search engine to retrieve similar sentences $\{\langle \boldsymbol{x}^r, \boldsymbol{y}^r\rangle\}$  from a bilingual database. Such a technique called {\bf translation memory} is helpful to improve the translation quality and efficiency for human translators~\cite{dillon2006translators}. As the development of machine translation techniques, there is a surge of interests in improving machine translation models with translation memory. In the rest of this section, we will review translation memory for both statistical machine translation (SMT) and neural machine translation (NMT). 

==> A Comprehensive Survey on Retrieval based Text Generation Methods/sec-other-tasks.tex <==


In addition to dialogue system and machine translation, retrieval-augmented generation techniques have shown to be beneficial in many other tasks. In the following, we highlight several key tasks that apply retrieval-augmented generation approaches.\footnote{Here, we focus on tasks other than question answering. We refer readers interested in QA to \citet{chen-yih-2020-open}.} % \hyli{Would it be better if we introduce the LM and summarization first? The order of those tasks in this section seems to be random.}

%are widely used in many other generation tasks as well. In the following, we highlight several key researches in different areas. 

\paragraph{Language Modelling} %Another line of research in retrieval-based text generation relates to general-domain language modelling. 
It has been shown that properly leveraging information from retrieval memory could improve the performance of large pre-trained language model. To build a more accurate language model, \citet{DBLP:conf/iclr/KhandelwalLJZL20} propose to incorporate a soft memory module into the system. Specifically, an index is built by caching the hidden states of the training corpus. Then, the language model accesses the index via k-NN search and displays a greatly improved performance. 
%proposed to use a pre-trained index as soft cache to implement k-NN based language model and observed greatly improved performance.
As another example, \citet{DBLP:journals/corr/abs-2002-08909} propose a new paradigm that applies retrieval-augmented technique into the pre-training of generative language model. During learning, they train a neural selector that dynamically samples a relevant text to guide the reconstruction of a corrupted input sequence. In this way, the pre-trained model delivers better results by explicitly grounding on the retrieval memory. \citet{DBLP:conf/nips/LewisGGAWZ20} combine language model pre-training with a paraphrasing approach. During learning, an input sequence to the model is first corrupted. In the meantime, a set of multi-lingual texts are retrieved based on which the model learns to reconstruct the original input sequence. 
%To reconstruct a target text, a set of related multi-lingual texts are first retrieved, based on which the model learns to reconstruct the original text \hyli{I cannot understand this}. 
Recently, \citet{DBLP:journals/corr/abs-2112-04426} propose \textsc{RETRO}, a large pre-trained language model enhanced with retrieved documents, and obtained comparable performances with GPT-3 using 25$\times$ fewer parameters.


\paragraph{Summarization} Text summarization is another research area that benefits from retrieval-augmented text generation. \citet{peng2019text} propose an adaptive decoding framework which first retrieves an exemplar document given the source document. Then, the summarization of the source document is derived through an adaptive generation process based on the retrieved template. Different from \citet{peng2019text}, \citet{DBLP:conf/acl/LiWLC18} and \citet{hossain2020simple} introduce an intermediate re-ranking stage into the generation pipeline. Specifically, before generating the document summary, the retrieval documents are first re-ranked based on their similarity scores with respect to the source document. Then, the document summarization is produced by re-writing the selected templates.



\paragraph{Paraphrase Generation} 
To address the lack of quality as well as diversity in the generation of paraphrases, \citet{kazemnejad-etal-2020-paraphrase} propose a generation framework which first retrieves a sentence that is similar to input sentence. Then, based on the retrieved sentence, a neural editor produces the resulting paraphrased sentence. \citet{DBLP:conf/acl/ChenTWG19} investigate a different aspect of paraphrasing, i.e. how to control the linguistic syntax displayed in the generated text. To achieve this goal, \citet{DBLP:conf/acl/ChenTWG19} propose to first extract a sentential exemplar that serves as the syntax template. A neural model then generates the paraphrase with desired linguistic syntax following the retrieved exemplar.

%The paraphrase is then produced by a neural model based on the extracted template. 






%\paragraph{Question Answering.} Retrieval-based text generation has also been shown to be useful in knowledge intensive tasks. \citet{DBLP:conf/nips/LewisPPPKGKLYR020} addressed the task of question answer by first building an neural document index from a  Wikipedia. Then, given a question, the neural indexer first retrieves a set of related documents based on which the generator generates the result. 

\paragraph{Text Style Transfer} To improve the quality of generated text, \citet{DBLP:conf/naacl/LiJHL18} propose a retrieval-augmented framework which first retrieves texts that are similar to the input based on lexical-level similarity. Then, the retrieved tokens that are irrelevant to the source are deleted, and the output is derived from the edited template. \citet{DBLP:conf/emnlp/XiaoPLWSC21} also adopte this framework by incorporating retrieval information from two sources (i.e. sparse and dense memories) and obtained an improved model performance. 


%This framework is also adopted by \citet{DBLP:conf/emnlp/XiaoPLWSC21} 



%in which an exemplar of the source document is first retrieved. Then, the generator adaptively produces the document summarization. \citet{DBLP:conf/acl/LiWLC18} and \citet{DBLP:conf/acl/HossainGZ20} address this task with a similar approach. Their approach differ from \citet{DBLP:conf/naacl/PengPFD019} in a way that, given the retrieved exemplar, the document summarization is produced via a re-rank and re-write process. 

\paragraph{Data-to-Text Generation} Recently, retrieval-augmented generation has been adapted to the task of data-to-text generation. To bridge the gap between the structured data and natural language text, \citet{DBLP:conf/emnlp/SuMBC21} propose a novel retrieval-augmented framework. Specifically, given the source data, a set of candidate texts are first retrieved from a large unlabelled corpus. Then, a neural selector is applied to measure the similarities between the source data and candidate texts, and extract a set of more fine-grained prototypes from the candidates. Lastly, a generation model takes the prototypes as input to produce the text that describes the given structured data.

%produce the output of the given structured data.

%proposed a retrieval-augmented framework which first selects a set of relevant texts from Wikipedia. The selected texts are then refined into more fine-grained prototypes using a neural selector. Lastly, a generation model takes the fine-grained prototypes as input to produce the output of the given structured data.

While retrieval-augmented generation has been widely explored in the NLP community, we suggest that future research could extend this approach to tasks that involve data from multiple modalities. For instance, with recent advancements in image-text retrieval  \cite{DBLP:conf/icml/JiaYXCPPLSLD21,DBLP:conf/icml/RadfordKHRGASAM21}, the structural gap between images and texts is largely bridged. Some early studies \cite{DBLP:conf/iclr/0001C0USLZ20} have shown that information retrieved from images could improve the performance of neural machine translation model. Naturally, such methods could be extended to other multi-modal tasks, such as image captioning \cite{DBLP:conf/cvpr/KarpathyL15}. %text-to-image generation \cite{DBLP:conf/icml/RameshPGGVRCS21}. 
A similar idea could also be applied to tasks beyond images, such as %text-to-speech synthesis \cite{DBLP:conf/ssw/OordDZSVGKSK16} and 
speech-to-text transcription \cite{DBLP:journals/ftsig/GalesY07}.









%\subsection{Task-Oriented Dialogue Generation}

%\subsection{Data-to-Text Generation}




==> A Comprehensive Survey on Retrieval based Text Generation Methods/sec-retrieval-paradigm.tex <==

\subsection{Formulation and Motivation}
Most text generation tasks can be formulated as a mapping from input sequence $\boldsymbol{x}$ to output sequence $\boldsymbol{y}: \boldsymbol{y} = f(\boldsymbol{x})$. For example, $\boldsymbol{x}$ and $\boldsymbol{y}$ could be the dialogue history and its response in dialogue generation, sequences in source language and target language in machine translation, and so on.
% For example, in dialogue generation $\boldsymbol{x}$ and $\boldsymbol{y}$ denote the dialogue history and response, respectively; in machine translation,  $\boldsymbol{x}$ and $\boldsymbol{y}$ are sequences in different languages with the same meaning; while in summarization a piece of long text $\boldsymbol{x}$ will be summarized to a short summary $\boldsymbol{y}$. 

% However, storing all necessary information in model parameters is inefficient, since it requires big memory and also results in high inference latency.

Recently, some researchers suggest to endow models the capability to access external memory via some information retrieval techniques, so that they can acquire more information in the generation process \cite{gu2018search, weston-etal-2018-retrieve, cai-etal-2019-retrieval}. The retrieval-augmented generation can be further formulated as:
\begin{equation}
    \boldsymbol{y} = f(\boldsymbol{x}, \boldsymbol{z})
\end{equation}
where $\boldsymbol{z} = \{\langle \boldsymbol{x}^r, \boldsymbol{y}^r\rangle\}$ is a set of relevant instances retrieved  from the original training set or external datasets. The main idea of this paradigm is that $\boldsymbol{y}^r$ may benefit the response generation, if $\boldsymbol{x}^r$ (or $\boldsymbol{y}^r$) is extremely relevant to the input $\boldsymbol{x}$. It is worth noting that $\boldsymbol{x}^r=\emptyset$ when unsupervised retrieval sources are used. More details about how to get $\boldsymbol{z}$ will be discussed in \cref{metrics}.

In this section, we will briefly introduce some basic IR techniques. In general, the retrieval memory can be retrieved from three kinds of sources: the training corpus, external datasets in the same format with the training corpus, and large-scale unsupervised corpus (\cref{sources}). Metrics that evaluate the relevance between text are varied as well, in \cref{metrics} we divided them into three categories: sparse-vector retrieval, dense-vector retrieval, and training-based  retrieval. Finally, how to integrate the retrieval memory to the generation model is also significant, we also introduce some popular integration approaches in  \cref{integration_fashion}.




\subsection{Retrieval Sources }
\label{sources}
Most previous studies search the external memory from its \textbf{training corpus}~\cite{song2016two, gu2018search, weston-etal-2018-retrieve}. In the inference time, retrieved examples with high relevant scores could be regarded as extra references and reduce model's uncertainty in generation. The main motivation of those works is to to store  knowledge not only in the model parameters but also in an explicit and accessible form, making the model be able to re-access it during inference.

Some researchers also propose to retrieval relevant samples from \textbf{external datasets} \cite{su2021prototype, DBLP:conf/emnlp/XiaoPLWSC21}. In these studies, the retrieval pool is different with the training corpus, which can further provide additional information that are not contained in the training corpus. This is especially beneficial for applications  such as domain adaptation and knowledge update. For example, \citet{khandelwal2020nearest,zheng2021adaptive} employ the in-domain dataset as the external memory to achieve fast domain adaptation for machine translation. 


One limitation for previous two sources is that the datasets have to be supervised datasets consisting of aligned input-output pairs. For machine translation, \newcite{cai-etal-2021-neural} propose a cross-lingual retriever to directly retrieve target sentence from \textbf{unsupervised} monolingual corpus. The main idea is aligning source-side sentences and the corresponding target-side translations in a dense vector space, i.e., aligning $\boldsymbol{x}$ and $\boldsymbol{y}^r$ when $\boldsymbol{x}^r$ is absent. As a result, the retriever directly connects the dots between the source-side input and target-side translations, enabling monolingual data in the target language to be used alone as memories.

\subsection{Retrieval Metrics}
\label{metrics}
Given an input sequence $\boldsymbol{x}$ and a retrieval corpus, retrieval model aims to retrieve a set of relevant examples $\boldsymbol{z} = \{\langle \boldsymbol{x}^r, \boldsymbol{y}^r\rangle\}$ from the corpus. When a supervised corpus is used, $\{\langle \boldsymbol{x}^r, \boldsymbol{y}^r\rangle\}$ is retrieved by measuring the similarity between $\boldsymbol{x}$ and $\boldsymbol{x}^r$.

For similarity measurement, \textbf{sparse-vector retrieval} methods such as TF-IDF and BM25~\cite{robertson2009probabilistic} are widely used. They match keywords efficiently with an inverted index. However, these methods prefer examples with similar surfaces, and may fail to retrieve examples that are only semantically relevant.

To alleviate above problem, some studies~\cite{cao-xiong-2018-encoding} attempt to retrieve in \textbf{dense-vector space} instead of the lexical overlap. Recent work \cite{lee2019latent} makes use of pre-trained language models, which encodes the text to low-dimensional dense vectors via BERT-based encoders. The retrieval score are computed via inner products between vectors.

Similarity-based retrieval is based on a simple heuristic. That is, the more $\boldsymbol{x}^r$ resembles with $\boldsymbol{x}$, the more likely $\boldsymbol{x}^r$ and $\boldsymbol{y}^r$ will help the generation. However, the most similar one by universal textual similarity does not necessarily serve the best for downstream models. Ideally, the retrieval metric would be learned from the data in a task-dependent way: we wish to consider a memory only if it can indeed boost the quality of final generation. \newcite{cai-etal-2021-neural} propose to unify the memory retriever and its downstream NMT model into a learnable whole. Such memory retrieval is end-to-end optimized for \textbf{task-specific} objectives. 
% \cd{I think the main strength of task-specific training is that task-specific relevance metrics perform better than the universal textual similarity. Note that task-specific metrics can also be used for supervised datasets while the textual similarity can also be used for unsupervised datasets}

\subsection{Integration}
\label{integration_fashion}
There are several ways to integrate the retrieved external memory in generation. One straightforward way is \textbf{data augmentation}, which constructs some augmented inputs by concatenating spans from $\{\langle \boldsymbol{x}^r, \boldsymbol{y}^r\rangle\}$ with the original input $\boldsymbol{x}$. By training on the augmented inputs, a generation model implicitly leans how to integrate the retrieved information.
Despite the simplicity, this kind of methods works efficiently in lots of tasks \cite{song2016two, weston-etal-2018-retrieve, bulte2019neural}.

% The most straightforward one is considering the retrieved results as auxiliary input and concatenate them with the model input \cite{song2016two, weston-etal-2018-retrieve}. In general, this 
% % However, due to the input length limit of generation model \cd{I do not think so}, one limitation for this concatenation-based integration method is that, in most cases, only one retrieved result can be integrated to the generation model.
% \hyli{Suggestion about the summary of data-augmentation methods: 1) simple and effective; 2) integration is in an implicit manner, and the model capacity doesn't increase}

% However, this integration method meets a serious issue that the generation 
% model may be degenerated to either a vanilla seq2seq model that ignore the retrieved results or a simple copy mechanism that simply take the retrieved result as the generation result. This phenomenon is caused by to the 1-to-n mapping problem in most generation tasks, where one input may correspond to multiple proper target sentences. The only way to alleviate this problem is putting hard constraints on the data so that the similarity between retrieved results and and the target sentence are neither too big nor too small, which greatly reduces the amount of usable data. 

Another integration method is based on the \textbf{attention mechanism} \cite{bahdanau2014neural}. The main idea of this fashion is adopting additional encoders (in various architectures) to encode retrieved target sentences, and integrate them through attention \cite{cao-xiong-2018-encoding, gu2018search, bapna2019non}. Since the attention mechanism is becoming \cite{bahdanau2014neural, vaswani2017attention} a key module in lots of NLP models, integrating retrieved memory through attention becomes a very nature and efficient way.  
% In machine translation \cd{also in other tasks}, some studies attending the retrieved results via the attention mechanism \cite{gu2018search}. They main idea is adopting additional encoders (in various architectures) to encode retrieved target sentences, and integrate them through attention mechanism \cite{cao-xiong-2018-encoding, gu2018search, bapna2019non}. Compared with the concatenating-based integration method, the main advantage of attention mechanism is it may utilize information from multiple retrieved results. \hyli{Disagree, lots of works in the data-augmentation fashion also concatenate multiple references with the input, which can also address the multi-reference problem.}

In previous two methods, an NLP model learns how to filter out irrelevant or even harmful information from the retrieved examples implicitly. There also exist some works that try to explicitly extract useful information, i.e., \textbf{skeleton extraction}, from the retrieved memory \cite{cai2019skeleton, wu2019response, cai-etal-2019-retrieval}. For example, one skeleton should be a part of a whole utterance with irrelevant content masked, and the generation model only integrate this skeleton in the generation process.

% In previous two methods, both proper content and improper content are integrated to the generation model, without any discrimination 
% %\hyli{I am not sure about this, because attention can also assign improper content with low attention scores.}
% . Some studies thus attempt to extract response skeleton/prototype from retrieved results \cite{cai2019skeleton, wu2019response, cai-etal-2019-retrieval}. Specifically, one skeleton should be a part of a whole utterance, with some improper content is masked. The generation model only integrate this skeleton into the the generation process, so that we can alleviate the effect of improper content in retrieved results to the generation result.




==> A Comprehensive Survey on Retrieval based Text Generation Methods/subsec-neural-machine-translation.tex <==
Translation memory has been widely explored in Neural Machine Translation (NMT). Depending on when retrieval is involved, we can categorize previous works into two classes: 1) an NMT model leans how to cooperate with the retrieval model in the training phase; 2) an NMT model is only aware of the retrieved data in the inference phase.

\paragraph{Inference Phase} The key point of literature in this line is to reward some target words based on words in $\boldsymbol{y}^r$ in the inference process. Thus, a decision can be made based on both the distribution of  generation model and the additional reward of retrieval model. Some previous works propose to reward target words based on the sentence-level similarity between $\boldsymbol{x}$ and $\boldsymbol{x}^r$, and the word alignment between $\boldsymbol{x}^r$ and $\boldsymbol{y}^r$. Given the input sentence $\boldsymbol{x}$, \citet{zhang2018guiding} try to assign target words in $\hat{\boldsymbol{y}}$ with higher rewards, when they appear in $\boldsymbol{y}^r$ and the aligned source words  are in both $\boldsymbol{x}^r$ and $\boldsymbol{x}$. \citet{he2019word} follow a similar framework and consider the position information of those target words when rewarding. Those works reward the target words in an explicit way, however, the one-sentence-one-model approach \cite{li2016one, turchi2017continuous} propose to reward target word implicitly. For each testing input $\boldsymbol{x}$, their approach will first finetune the translation model on retrieved memory $\{\langle\boldsymbol{x}^r, \boldsymbol{y}^r\rangle\}$ and then translate $\boldsymbol{x}$.

Others try to reward target words based on token-level similarity score. Most works in this line are based on the dense retriever~\cite{khandelwal2020nearest}, e.g., faiss. \citet{khandelwal2020nearest} build a key-value datastore, where key $h(\boldsymbol{x}^r, \boldsymbol{y}^r_{<t})$ is the hidden state at each time step when translating $\boldsymbol{y}^r$ from $\boldsymbol{x}^r$, and value is its golden-truth target word $\boldsymbol{y}^r_{t}$. Therefore, in the inference time, they can use the $h(\boldsymbol{x}, \hat{\boldsymbol{y}}_{<t})$ as query and reward target words with similar hidden representations in the datastore. Although this method achieves significant performance gain, one drawback of it is the high latency. To address this issue, \citet{meng2021fast} use some heuristics, e.g., pre-filtering, to avoid searching on the entire datastore. The reward score of previous works is got from some non-parametric approaches, however, \citet{zheng2021adaptive} propose a light-weight network to learn the reward score. Since dense retrieval has the potential of cross-lingual retrieval, \citet{zheng2021non} use a similar approach to achieve unsupervised domain adaptation, where a main change is to create the datastore based on synthetic sources sentence and the real target sentences.

% A big advantage of those approach is that they do not need to change the architecture or parameters of the generation model, making it very flexible.

\paragraph{Training Phase} Different from those model-agnostic approaches, previous works in this line aim to train the generation model to learn how to cooperate with the retrieval model. It is also worth noting that most works in this line adopt the sentence-level retrieval, when integrating the retrieval information in the training process. To achieve its goal, \citet{bulte2019neural} and \citet{hossain2020simple} propose a data augmentation method to integrate the retrieved information, where $\boldsymbol{x}$ is concatenated with $\boldsymbol{y}^r$ before feeding into the model . Following the data augmentation approach, \citet{xu2020boosting} propose more matching methods to determine including which retrieved example in the source is better. 

There also exist some works that propose new architectures to integrate the retrieval information. Under the RNN-based framework, \citet{cao-xiong-2018-encoding} and \citet{gu2018search} use the gating and attention mechanism to incorporate the retrieved target sentences. When Transformer \cite{vaswani2017attention} becomes the backbone of NMT, some works also use additional transformer encoders to encode retrieved target sentences, and integrate them through attention mechanism \cite{bapna2019non, cao2019learning}. \citet{xia2019graph} represent the retrieved target sentences in a different data structure, i.e., a graph structure, and integrate it through attention mechanism. \citet{he2021fast} propose a light-weight method to encode the retrieved target sentences and leverage the alignment information to filter out irrelevant information. Different from previous works that rely on bilingual memories, \citet{cai-etal-2021-neural} propose a framework that can retrieve the most similar target sentence in a monolingual dataset, using a source sentence as query.

\paragraph{Limitations} In the section of SMT, we have showed some limitations of the retrieval augmented approaches. There also exist some limitations in the line of NMT. First, the information used for deriving reward scores is limited. The similarity between an input and retrieved examples is the primary feature to derive reward scores. However, some information, e.g., frequencies of words and context, may also be beneficial for integrating the translation memory. Second, it remains to be an open question that when should we use the retrieved information and when not. In the inference phase, approaches tend to integrate the translation memory excessively, e.g., at each time step, which not only reduces the translation efficiency but may also dampen the fluency of generated results.






==> A Comprehensive Survey on Retrieval based Text Generation Methods/subsec-statistical-machine-translation.tex <==

Generally, SMT includes three key components in a pipeline manner such as phrase table extraction, parameter tuning and decoding~\cite{koehn-etal-2003-statistical,chiang2007hierarchical}. As a result, many efforts have been made to make use of translation memory (TM) on top of each component. 

\paragraph{Constrained Decoding with TM}
Constrained decoding is the most straightforward way to integrating TM into SMT~\cite{smith2009ebmt,koehn2010convergence,zhechev2010seeding,ma2011consistent}. Its basic idea is to reuse the useful segments 
in $\boldsymbol{y}^r$ while translate other segments by SMT. Specifically, the approach consists of three steps: 1) identify the unmatched segments in both $\boldsymbol{x}^r$ and $\boldsymbol{x}$ through the edit-distance algorithm; 2)
identify the unmatched segments in $\boldsymbol{y}^r$, each of which is aligned to one unmatched segment in $\boldsymbol{x}^r$ by a word alignment algorithm; 3) decode each unmatched segment in $\boldsymbol{x}$ by SMT and then use the result to replace its corresponding unmatched segment in $\boldsymbol{y}^r$. \citet{li2016phrase} further extend this approach from sentence level to phrase level. 
The advantage in constrained decoding is that it does not require to change the translation model (including phrase table and parameters) and can be applied in a plug-and-play way. 
This approach is successful when $\boldsymbol{x}$ is highly similar to $\boldsymbol{x}^r$; otherwise its performance is degraded largely, because it explicitly isolates TM matching and SMT decoding and reuses the results in $\boldsymbol{x}^r$ or not in a deterministic way.  

\paragraph{Phrase Table Aggregation with TM}
There are also notable efforts to augment the phrase table for SMT by extracting translation rules from the retrieved bilingual sentences $\{\langle\boldsymbol{x}^r, \boldsymbol{y}^r\rangle\}$. Then they re-tune the parameters for the SMT model which makes use of translation knowledge from $\{\langle\boldsymbol{x}^r, \boldsymbol{y}^r\rangle\}$ in a implicit way when translating $\boldsymbol{x}$. For example, \citet{biccici2008dynamic,simard2009phrase} directly combine the extracted translation rules into the phrase table in a shallow combination way. They introduce an additional feature to indicate that whether translation rule is from $\{\langle\boldsymbol{x}^r, \boldsymbol{y}^r\rangle\}$ or not and then train all feature weights with MERT~\cite{och-2003-minimum}. One characteristic of these work is that a translation rule extracted from $\{\langle\boldsymbol{x}^r, \boldsymbol{y}^r\rangle\}$ which can not exactly match any segments in $\boldsymbol{x}$ is useless even if it may contain some useful words in its target side. To remedy this observation, \citet{wang2013integrating,wang2014dynamically} resort to a deep combination way to using the extracted translation rules. For each rule in the phrase table, it designs a generative model to reward the rules which are similar to those extracted from $\{\langle\boldsymbol{x}^r, \boldsymbol{y}^r\rangle\}$. Then this generative model is used as a feature in the log-linear based SMT model whose weight is tuned together with other features by MERT. In addition, \citet{li2014discriminative} employ a similar way to reward the rules but it relies on a discriminative model which is easy to integrate potential features from $\{\langle \boldsymbol{x}^r, \boldsymbol{y}^r\rangle\}$. 

\paragraph{Parameter Tuning with TM}
Unlike the above two research lines, 
\citet{liu2012locally,liu2014discriminative} make use of translation memory only in tuning parameters. To be specific, when translating an input sentence $\boldsymbol{x}$, they firstly retrieve many similar bilingual sentences $\{\langle \boldsymbol{x}^r, \boldsymbol{y}^r\rangle\}$, and then tune the  parameters on top of the retrieved sentences as well as a given development dataset in a sentence-wise manner, i.e., it performs an independent tuning for each input sentence. To improve the efficiency of each tuning step, it propose a local update on top of $\{\langle \boldsymbol{x}^r, \boldsymbol{y}^r\rangle\}$ from a baseline model.  

% \paragraph{Others}

Despite the successes of translation memory in SMT, there are still some limitations for the above three kinds of methods. Firstly, all these methods employ fuzzy score for retrieval which is highly dependent on word matching and thus can not recall such examples which are similar in word semantics but different in surface form. Secondly, these methods integrate the retrieved examples into a module of SMT in the ways which can not make full use of the knowledge in retrieved examples. For example, the integration ways in the first two kinds (constrained decoding and phrase table aggregation) are heuristic and not optimized towards translation quality; the parameter tuning method fine-tunes few parameters for log-linear based SMT which are not enough to preserve sufficient knowledge from retrieved examples. 
Thirdly, since SMT performs in a pipeline manner, it is intractable to jointly optimize retrieval metrics as well as SMT models. Consequently, all these methods adopt an off-the-shelf metric for retrieval, leading to sub-optimal performance. 


